Optimal Learning of Specifications from Examples

A fundamental challenge in synthesis from examples is designing a learning algorithm that poses the minimal number of questions to an end user while guaranteeing that the target hypothesis is discovered. Such guarantees are practically important because they ensure that end users will not be overburdened with unnecessary questions. We present SPEX -- a learning algorithm that addresses the above challenge. SPEX considers the hypothesis space of formulas over first-order predicates and learns the correct hypothesis by only asking the user simple membership queries for concrete examples. Thus, SPEX is directly applicable to any learning problem that fits its hypothesis space and uses membership queries. SPEX works by iteratively eliminating candidate hypotheses from the space until converging to the target hypothesis. The main idea is to use the implication order between hypotheses to guarantee that in each step the question presented to the user obtains maximal pruning of the space. This problem is particularly challenging when predicates are potentially correlated. To show that SPEX is practically useful, we expressed two rather different applications domains in its framework: learning programs for the domain of technical analysts (stock trading) and learning data structure specifications. The experimental results show that SPEX's optimality guarantee is effective: it drastically reduces the number of questions posed to the user while successfully learning the exact hypothesis.

==> algorithm.tex <==
\section{Exploring the Space of Programs} 

\subsection{High Level Algorithm}

\subsection{CEGIS Instantiation}

==> background.tex <==
\section{Technical Analysis Background}\seclabel{background}
%In this section we provide the background for our work, starting from technical analysis, proceeding to concept learning and active learning.

%\subsection{Technical Analysis}
In this section, we provide a background on technical analysis.
Technical analysis is a methodology aiming to predict stock price direction (\emph{trend}) based on the available price information~\cite{Murphy:TABook}, such as the stock price, volume, and open interest. Technical analysts use charts to capture this information and to forecast new trends. 

Technical analysts believe that any factor affecting the price (e.g., political factors) is reflected in the price chart, and thus studying the price chart provides as much information as required to predict the price trend. In addition, analysts believe that prices move in trends, and their goal is to identify trends at early stages.

An advantage of the technical analysis approach over other price prediction approaches is its ability to cope simultaneously with multiple stocks. Technical analysis requires no knowledge of the stocks, and thus analysts may track multiple stocks simultaneously and focus their attention to stocks showing interesting trends.

\para{Line Charts}
We focus on \emph{line charts} which present the line connecting the daily closing prices (e.g.,~\figref{line_chart}). Many analysts believe that the closing price is the most significant indicator of the price activity, and thus believe that line charts are more indicative to measure this activity than other chart types. In fact, Dow, whose theory is considered as one of the technical analysis origins, used only the closing stock prices as buy and sell signals. We use the \emph{arithmetic} chart scale in which the distance between data points is equal.
\ignore{
\begin{figure}
 \includegraphics[width=0.48\textwidth,clip=true,trim=0pt 0pt 0pt 0pt]{figures/apple_chart_example.png}
 \caption{A line chart of AAPL stock price.}
 \figlabel{line_chart}
\end{figure}}

\para{Trends}
There are three trend directions, \emph{uptrend}, \emph{downtrend}, and \emph{sideways trend}. However, stock prices do not move in a straight line in any trend direction, but rather in zigzags (see~\figref{line_chart} for example). Thus, the stock trend is determined based on the notable peak and low points. For example, uptrend is characterized by a sequence of peaks each higher than its previous (e.g., the prices between May 14 and September 14 in~\figref{line_chart} show an uptrend).

\para{Patterns} Changes in price trends are usually not swift and last for a certain period. The challenge is to quickly detect that a change has begun to enable fast response (selling or buying). To this end, analysts search for \emph{patterns} in the chart. Patterns are formulations which usually occur under certain conditions, and thus assist in predicting future trends.

Pattern formulations consist of several consecutive trends and can be described by the points connecting adjacent trends.
For example, the head and shoulder pattern (\figref{HeadShoulders}) takes the form of three consecutive occurrences of an uptrend followed by a downtrend, and it is described by the relationships between points connecting uptrends with downtrends (the red rectangles in~\figref{HeadShoulders}). The relationship between two adjacent points captures the trend between these two points. For example, in the head and shoulder pattern, the first point is smaller than the second point, implying this pattern begins with an uptrend.

\ignore{There are two main types of patterns, \emph{reversal} and \emph{continuation}. Reversal patterns indicate that the trend is reversed, and continuation patterns indicate that the trend has paused but will resume. Since reversal patterns often require a response, they are classified as \emph{major}, whereas continuation patterns are classified as \emph{intermediate} or \emph{minor}.}

The literature presents several patterns, which are well-known and often assist in prediction. However, these theoretical patterns occur little in the inspected data. Thus, analysts consider \emph{pattern variations}, namely, formulations which are similar to the theoretical patterns with a few changes. \tool's task is to assist analysts with learning patterns, adjusting them to their needs, and update them if the real world data observe too little or too many occurrences of the pattern.


\ignore{\subsection{SMT-Solvers}
SMT-solvers address the challenge of finding whether a first-order logical formula is satisfiable. In this work, we use the~\emph{Z3} SMT-solver~\cite{DeMoura:2008}. Though addressing any first-order logical formula is still under ongoing research, \emph{Z3} is very efficient in checking satisfiability of formulas without quantifiers and function symbols.

If a formula is found to be satisfiable, \emph{Z3} provides a satisfying assignment. If a formula is unsatisfiable, \emph{Z3} produces an \emph{unsat core}. An unsat core is a set of clauses causing the formula to be unsatisfiable. Namely, if they will be removed from the formula, it will be satisfiable. A \emph{minimal unsat core} is an unsat core which is minimal, namely, any strict subset is not an unsat core. Alternatively, removing strict subsets of a minimal unsat core results in an unsatisfiable formula.}

\ignore{
\subsection{Problem Setting}
We focus on the prices of a single stock, which are assumed to arrive one after the other in a
stream-fashion.
At each point of time, we focus on a fixed-size sequence of prices, which we refer to as
\emph{a window}. Upon the arrival of a new point, the oldest point is omitted and the new one is
added to the observed window. This is often referred to as a \emph{sliding
window}~\citep*{Datar:2002}.
We limit the search of patterns to the points inside a window. As a result, we miss occurrences
of a pattern that span multiple windows. There is a known tradeoff between the size of the
sliding window (allowing the detection of wider patterns) and the performance of pattern
detection.

\subsubsection{Challenges in Detecting Patterns}
Several challenges arise when attempting to detect patterns in windows.

\paragraph{Unclear Characterization of the Pattern}
The descriptions presented above were taken from technical analysts books
\citep*{Murphy:TABook}. The descriptions of all patterns is somewhat vague. For
example, consider the {\cupnh} pattern. The pattern does not specify the
depth of the cup, what is a minor descent, and so on. To illustrate the
challenge in such description, consider the two charts
in~\figref{challenge-cupnhandle}. Both charts appear to follow the {\cupnh}
description, however it is not clear whether \figref{challenge-cupnhandle}(b)
should be considered as match for this pattern.

\begin{figure}
\centering
\begin{tabular}{cc}
\includegraphics[width=.222\textwidth,clip=true]{figures/challenge_cupnhandle2.png} &
\includegraphics[width=.222\textwidth,clip=true]{figures/challenge_cupnhandle1.png} \\
(a) & (b)
\end{tabular}
    \caption{Candidates for the {\cupnh} pattern: (a) follows the exact description; (b) is a
    variation.}
    \figlabel{challenge-cupnhandle}
\end{figure}



\paragraph{Noise in the Data}
A stock's price chart is not a smooth graph, and as such it may be exposed to
momentarily spikes. When a human analyst inspects such spikes, she can
(usually) distinguish between a spike which is a noise and an important
spike. One approach to handle such noise is by smoothing the chart (e.g.,
using~\citep*{Schafer:IEEE11}). There are many smoothing techniques, each has
characteristics that are preserved, and information that is
lost~\citep*{DSPBook}. Thus, it may be the case that different patterns require
different smoothing techniques. In addition, the loss of information can have
a dramatic impact on the shape of a chart. For example, consider the charts
of~\figref{challenge-noise}, where~\figref{challenge-noise}(a) represents
the raw data, and of~\figref{challenge-noise}(b) represents the smoothed
data. In~\figref{challenge-noise}(a), there is a distinct low, whereas, in
of~\figref{challenge-noise}(b) this low seems less significant. It is not
clear if the loss of information can result in missing matches of patterns.
\begin{figure}
    \centering
    \begin{tabular}{cc}
  \includegraphics[width=.222\textwidth,clip=true]{figures/challenge_noise1.png} &
    \includegraphics[width=.222\textwidth,clip=true]{figures/challenge_noise2.png} \\
    (a) & (b)
    \end{tabular}
  \caption{The effect of smoothing data: (a) the raw data, and (b) the smoothed data.}
    \figlabel{challenge-noise}
\end{figure}
%\paragraph{The shrinkage/ expenditure}\TODO{}
%\paragraph{Bias in Shapes}\TODO{}

}


==> cnf-form.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
%rem = $S \setminus (S_{N}\cup Rs)$\;
%\Return{$S_{P}\cup Rs \cup \{\neg r \mid r\in S \setminus (S_P \cup S_{N}\cup Rs)\}$}
\Return{$\bigwedge_{Q\in Rs} Q \wedge \bigwedge_{Q\in S_{0} \setminus Rs} \neg Q$}
\caption{CNF-form($Rs$,$S_{0}$,$S_N$)}\funlabel{cnfform}
\end{function}


==> cnf-implied.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
\Return{$\{\hat{l^{cl}}\mid \bigvee_{q \in S_P \cup \{l^{cl}\}} q \models \hat{l^{cl}}\}$}
\caption{CNF-implied($S_P$,$l^{cl}$)}\funlabel{cnfimp}
\end{function}

==> cnf-init.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
\Return{$\bigwedge_{e \in E_N} [\bigvee_{l \in S : e\models l} \neg l]$}
\caption{D-init($S$,$E_N$)}\funlabel{cnfinit}
\end{function}


==> code-conjunctivevar.tex <==

\begin{figure*}[h!]
%\begin{adjustwidth*}{-0.2cm}{-0.2cm}
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\input{con-init}
\end{minipage} \null
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\input{cnf-init}
\end{minipage}
%\end{adjustwidth*}%\vspace{-0.4cm}
%\begin{adjustwidth*}{-0.2cm}{-0.2cm}
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\input{con-form}
\end{minipage} \null
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\input{CNF-form}
\end{minipage}

\begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\input{con-implied}
\end{minipage} \null
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\input{cnf-implied}
\end{minipage}

%\begin{adjustwidth*}{-0.2cm}{-0.2cm}
\begin{comment}
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
allNeg = true\;
\For {$(Rs,\hat{e}) \in Examples$}{
    \If{$\exists e' \in E_N^u$:$e' \equiv \hat{e}$ $||$ ask($\hat{e}$)$=$n}{ $E_N^u$ = $E_N^u \cup \{\hat{e}\}$; continue}
     $S_{N} = S_{N} \cup Rs$\lnlabel{learnPos}\;
     $\varphi_{lb}$ = $\varphi_{lb} \setminus \{R^{cl} \mid R^{cl}\in Rs\}$\;
      allNeg = false\; break\;%

    }
\If{allNeg}{
    $S_{P} = S_{P} \cup$ $\{\hat{R}^{cl}  \mid S_P \cup \{R\} \models \hat{R}^{cl}\}$\;   \lnlabel{nextpredImplied}
}

\caption{Con-classify()}\funlabel{conclass}
\end{function}
\end{minipage} \null
 \begin{minipage}{6.05cm}
\null
\removelatexerror% Nullify \@latex@error
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
allPos = true\;
\For {$(Rs,\hat{e}) \in Examples$}{
    \If{$\exists e' \in E_P^u$:$e' \equiv \hat{e}$ $||$ ask($\hat{e}$)$=$p}{$E_P^u$ = $E_P^u \cup \{\hat{e}\}$; continue}
     $S_{N} = S_{N} \cup Rs$\lnlabel{learnPos}\;
     $\varphi_{lb}$ = $\varphi_{lb} \setminus \{R^{cl} \mid R^{cl}\in Rs\}$\;
      allPos = false\; break\;%

    }
\If{allPos}{
    $S_{P}$$=$$S_{P}$$\cup$ $\{\hat{R}^{cl}$$\mid$$\bigvee_{q^{cl} \in S_P \cup \{R^{cl}\}} q^{cl}$$\models$$ \hat{R}^{cl}\}$\lnlabel{nextpredImplied}
}
\caption{CNF-classify()}\funlabel{cnfclass}
\end{function}
\end{minipage}
%\end{adjustwidth*}%\vspace{-0.4cm}

\end{adjustwidth*}
\end{comment}
\end{figure*}




==> con-form.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
%rem = $S \setminus (S_{N}\cup Rs)$\;
\Return{$\bigwedge_{Q\in Rs} \neg Q \wedge \bigwedge_{Q\in S_{0} \setminus (S_{N}\cup Rs)} Q$}
\caption{C-form($Rs$, $S_{0}$, $S_N$)}\funlabel{conform}
\end{function} 

==> con-implied.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
\Return{$\{\hat{l} \mid \bigwedge_{q \in S_P \cup \{l\}} q  \models \hat{l}\}$}
\caption{C-implied($S_P$,$l$)}\funlabel{conimp}
\end{function} 

==> con-init.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
%\Return{$\bigwedge_{l \in S : \forall e\in E_P. e\models l} l$}
\Return{$\{l \in S \mid \forall e\in E_P. e\models l \}$}
\caption{C-init($S$,$E_P$)}\funlabel{coninit}
\end{function} 

==> d-form.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
%rem = $S \setminus (S_{N}\cup Rs)$\;
%\Return{$S_{P}\cup Rs \cup \{\neg r \mid r\in S \setminus (S_P \cup S_{N}\cup Rs)\}$}
\Return{$\bigwedge_{Q\in Rs} Q \wedge \bigwedge_{Q\in S_{0} \setminus (S_{N}\cup Rs)} \neg Q$}
\caption{D-form($Rs$,$S_{0}$,$S_N$)}\funlabel{dform}
\end{function}


==> d-implied.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
\Return{$\{\hat{l}\mid \bigvee_{q \in S_P \cup \{l\}} q \models \hat{l}\}$}
\caption{D-implied($S_P$,$l$)}\funlabel{dimp}
\end{function} 

==> d-init.tex <==
\begin{function}[H]
\small
\DontPrintSemicolon
\LinesNumbered
%\Return{$[\bigvee_{l \in S : \forall e \in E_N. \models l} \neg l]$}
\Return{$\{\neg l \in S \mid \forall e \in E_N. e \models l\}$}
\caption{D-init($S$,$E_N$)}\funlabel{dinit}
\end{function} 

==> detection-algo.tex <==
\section{Detecting Patterns in Streams}\seclabel{detect}

In this section, we describe how to detect patterns in stock streams, given a pattern formula $\varphi_P$.

As discussed in~\secref{eval}, the stream is inspected using a sliding window which reads fixed portions of the stream one by one. The formal definition of a window is identical to chart, thus given a window $w$ and a pattern of size $n$ captured by the formula $\varphi_P$, the window is a pattern occurrence if $w \models \varphi_{detect}$, where:
\[\varphi_{detect} = \exists {i_0},...,{i_{n-1}}. \varphi_P(w({i_0}),...,w({i_{n-1})})\]

and $w(j)$ is the price at time point $j$.

As discussed in~\secref{newformal}, the points should hold: $0 \leq i_0$$<$$i_1$$<$$\dots$$<$$i_{n-1}$$<$$|w|$. These constraints are encoded to a formula which is added to $\varphi_{detect}$:
\[
\begin{array}{l}
\varphi_{s}(i_0,...,i_{n-1}) = 0\leq i_0 \wedge i_{n-1}$$<$$|w| \wedge
 \underset{0 \leq j < n-1}{\bigwedge}  i_j$$<$$i_{j+1}
\end{array}
\]

As before, we wish to use the \emph{Z3} SMT-solver to check satisfiability. To this end, several adjustments are required.

\para{Encoding Windows into the Formulas}
As discussed in~\secref{newformal}, a window is a function mapping time points to their corresponding price points.
Since functions cannot be encoded explicitly in formulas, the function symbols $w({i_0}),...,w({i_{n-1}})$ are encoded to free variables, $p_0,...,p_{n-1}$. To ensure these variables are assigned the correct price values, $\varphi_{detect}$ is extended with additional constraints.

For each variable $p_j$ the following constraint is added:
$$\varphi_{price}(i_j, p_j) =  \underset{0 \leq l \text{\lt} |w|}{\bigwedge}  i_j = l \implies p_{j} = w(l)$$
whose interpretation is: if $i_j$ is assigned to the time point $l$, then $p_j$ is assigned to $w(l)$. Since $i_j$ value lies between $0$-$|w|$, $p_j$ is guaranteed to have a valid price point.
%The formula enforces to assign the correct price point if $i_j$ is assigned a value $l$. Since $i_j$ can be assigned any value between $0-|w|$ (where $|w|$ is the window size), a set of constraints is added to ensure that regardless of $i_j$ value, $i_j$ and $p_j$ capture time-point and its matching price-point in the given window. This is captured by the conjunction:
This constraint is added for all these new variables, resulting in the formula:
\[
\begin{array}{l}
\varphi_{prices}(i_0,...,{i_{n-1}},p_0,...,p_{n-1}) = \underset{0 \leq j \text{\lt} n-1}{\bigwedge} \varphi_{price}(i_j,p_j)
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \underset{0 \leq j \text{\lt} n-1}{\bigwedge}[\underset{0 \leq l \text{\lt} |w|}{\bigwedge}  i_j = l \implies p_{j} = w(l)]
\end{array}
\]
%{\[
%\begin{array}{l}
%     \exists {i_0},...,{i_{n-1}},p_0,...,p_{n-1}. \\
%     ~~~~~~~~~~~~~~~~~~~\varphi_P(p_0,...,p_{n-1}) \wedge \underset{0 \leq j \text{\lt} n-1}{\bigwedge}  i_j \text{\lt} i_{j+1}\wedge\\ \\
%     ~~~~~~~~~~~~~~~~~~~ (0\leq i_0) \wedge (i_{n-1} \leq |w|) \wedge \\ \\
%     ~~~~~~~~~~~~~~~~~~~ ]
%\end{array}
%\]
%}

\para{Stock Price Equality}
Stock prices are equal if their values are close compared to the nearby prices. For example, in~\figref{HeadShoulders}, the prices on dates October $14^{th}$ and $15^{th}$ are considered equal. Thus, the relation $\ltpred{}{}$\, is encoded as follows:
\vspace{-0.1cm}
\[
\ltpred{p_i}{p_j} \Leftrightarrow p_i + k_{Eq} \cdot 0.01 \cdot avg(w) < p_j
\vspace{-0.1cm}
\]
Namely, $p_i$ is less than $p_j$ if its value plus $k_{Eq}$\% of the average price in the window are less than $p_j$, where $k_{Eq}$ is a parameter configured by the user.

\para{Encoding Trends}
%The formula as stated above can be used to detect patterns of size $n$ in windows of size at least $n$. In windows whose size is greater than $n$, not only is it required to select $n$ points for satisfying the pattern formula, but also the unselected points in the window are required to meet some conditions.
%
As discussed in~\secref{newformal}, patterns consist of consecutive trends and are described by the relationships between the points connecting two adjacent trends. In~\secref{algo}, {\tool} learned the relationship between these points, but to capture the actual pattern, the trends must be encoded into $\varphi_{detect}$.
The trend definition may vary between analysts, but consist of similar ingredients, which we next present.

\para{Width of Trend} Typically, two consecutive points are not considered a trend, and a minimal number of points should appear between them in order that they will be considered to represent one.
Similarly, the maximal number of points between two time points representing a trend can be defined. These constraints are encoded as follows:
$$\varphi_{width}(i_0,...,{i_{n-1}}) = \underset{0 \leq j \text{\lt} n-1}{\bigwedge} k_{min} < (i_{j+1} - i_{j}) < k_{max}$$ where $k_{min}, k_{max}$ are parameters indicating the minimal and maximal number of points between adjacent time points.

\para{Trend Types} The relationship between two adjacent time points determines the trend of points lying between them, which is \emph{uptrend}, \emph{downtrend}, or \emph{sideways}. For example, if $p_j$$<$$p_{j+1}$, then for every $k \in (i_{j},i_{j+1})$, its price, $w(k)$, should follow the trend, namely, $p_j$$<$$w(k)$$<$$p_{j+1}$.
%For example, consider the chart in~\figref{HeadShoulders} reflecting the head and shoulder pattern. In this chart, the first rectangle point is lower than the second rectangle point, implying that all points between them should respect this uptrend.

However, stock prices are not smooth functions, and thus an uptrend is rarely one where each point is higher than its previous one; similarly downtrend and sideways trend may hold even if the mathematical definition does not.
Thus, we rely on the next definition of when a trend is followed, and note that alternative definition may be substituted for it.
  A trend is followed between $i_j$ and $i_{j+1}$ if the following holds:
  \begin{itemize}[nosep,noitemsep]
    \item For all $k \in (i_{j},i_{j+1})$, the price of $k$ lies between the prices of $p_j$ and $p_{j+1}$, which is encoded as follows: %Namely, for an uptrend:
         \[
         \begin{array}{l}
    \varphi_{up}(i_j, p_j, k)=\ltpred{p_j}{p_{j+1}} \implies  \ltpred{p_j}{w(k)} \wedge \ltpred{w(k)}{p_{j + 1}}\\\\
    \varphi_{dn}(i_j, p_j, k)=\ltpred{p_{j+1}}{p_{j}} \implies  \ltpred{p_{j+1}}{w(k)} \wedge \ltpred{w(k)}{p_{j}}\\\\
    \varphi_{sd}(i_j, p_j, k)=\neg (\ltpred{p_j}{p_{j+1}}) \wedge \neg (\ltpred{p_{j}}{p_{j+1}}) \implies \\
     ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \neg (\ltpred{p_j}{w(k)}) \wedge \neg (\ltpred{w(k)}{p_{j+1}})
     \end{array}
    \]
%     for a downtrend:
%     and for a sideways-trend:
Then, we define the trend formula, added to $\varphi_{detect}$:
\[
\begin{array}{l}
\varphi_{trend}(i_0,...,{i_{n-1}},p_0,...,p_{n-1}) = \\
\underset{0 \leq j \text{\lt} n-2}{\bigwedge}[\underset{0 \leq l \text{\lt} |w|}{\bigwedge} (i_j < k < i_{j+1}) \implies (\varphi_{up}(i_j,p_j,k) \wedge \\
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\varphi_{dn}(i_j,p_j,k) \wedge \varphi_{sd}(i_j,p_j,k))]
\end{array}
\]
\item If $i_j$ and $i_{j+1}$ represent an uptrend, then there are no $k_{Trnd}$ consecutive points forming a downtrend between them; similarly, if these points represent a downtrend, there are no $k_{Trnd}$ consecutive points forming an uptrend between them. $k_{Trnd}$ is configured by the user. These constraints are encoded similarly to previous constraints.
  \end{itemize}
%Thus, each pattern formula is extended to verify that points between the selected points follow the trend.
%Given three price points $p_i$, $p_k$, $p_j$, the trend formula $\varphi_{up}$ is defined as follows:
%$$\varphi_{up}(p_i,p_j,p_k)=\ltpred{p_i}{p_{j}} \implies \ltpred{p_i}{w(k)} \wedge \ltpred{w(k)}{p_{j}}$$
%the meaning of the formula is that if there is an uptrend from $p_i$ to $p_j$, then $w(k)$ follows this trend, and is greater than $p_i$ and smaller than $p_j$. Note that we do not compare points lying between $p_i$ and $p_j$ to themselves, as the trend is not smooth but rather continues in zigzag. Thus, it is possible that even though the overall line chart shows an uptrend between $p_i$ and $p_j$, in between there are zigzags.

%Similarly, we define the $\varphi_{down}$, and $\varphi_{sideways}$ formulas:

%$$\varphi_{down}(p_i,p_j,p_k)=\ltpred{p_{j}}{p_{i}} \implies \ltpred{p_{j}}{w(k)} \wedge \ltpred{w(k)}{p_{i}}$$
%{\[
%\begin{array}{l}
%     \varphi_{sideways}(p_i,p_j,p_k)=\neg (\ltpred{p_i}{p_{j}}) \wedge \neg (\ltpred{p_{j}}{p_{i}})\implies \\
%     ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\neg (\ltpred{p_i}{w(k)}) \wedge \neg (\ltpred{w(k)}{p_{j}})
%\end{array}
%\]
%}

%The trend formula is defined over two selected consecutive points $i_j$, $i_{j+1}$ and a point $k$, and if $k$ lies between $i_j$ and $i_{j+1}$, then the formula is satisfiable only if $k$'s price follows the trend between the prices of $i_j$ and $i_{j+1}$:
\ignore{
{\[
\begin{array}{l}
     \varphi_{trend}(i_j, i_{j+1}, k) = i_j < k \wedge k < i_{j+1} \implies \\
     ~~~~~~~~~~~~~~~~~~~~~~~~~~~~[\varphi_{up}(p_j, p_{j+1},w(k)) \wedge \\
     ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\varphi_{down}(p_j, p_{j+1},w(k)) \wedge \\
     ~~~~~~~~~~~~~~~~~~~~~~~~~~~~\varphi_{sideways}(p_j, p_{j+1},w(k))]

\end{array}
\]
}
And thus the overall trend formula:
\[
\begin{array}{l}
\varphi_{trends}(i_0,...,{i_{n-1}},p_0,...,p_{n-1}) = \\
     ~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \underset{0 \leq j \text{\lt} n-2}{\bigwedge}[\underset{0 \leq l \text{\lt} |w|}{\bigwedge}  \varphi_{trend}(i_j,i_{j+1},l)]
\end{array}
\]

This constraint is added for each triplet, resulting in the extended formula:
{\[
\begin{array}{l}
     \varphi_{detect}(w) = \exists {i_0},...,{i_{n-1}},p_0,...,p_{n-1}. \\
     ~~~~~~~~~~~~~~~~~~~\varphi_P(p_0,...,p_{n-1}) \wedge \varphi_{series}(i_0,...,{i_{n-1}})\wedge \\ ~~~~~~~~~~~~~~~~~~~\varphi_{prices}(i_0,...,{i_{n-1}},p_0,...,p_{n-1}) \wedge \\ ~~~~~~~~~~~~~~~~~~~\varphi_{trends}(i_0,...,{i_{n-1}},p_0,...,p_{n-1})
\end{array}
\]
}
}

\ignore{{\[
\begin{array}{l}
     \exists {i_0},...,{i_{n-1}},p_0,...,p_{n-1}. \\
     ~~~~~~~~~~~~~~~~~~~\varphi_P(p_0,...,p_{n-1}) \wedge \underset{0 \leq j \text{\lt} n-1}{\bigwedge}  i_j \text{\lt} i_{j+1}\wedge\\ \\
     ~~~~~~~~~~~~~~~~~~~ (0\leq i_0) \wedge (i_{n-1} \leq |w|) \wedge \\ \\
     ~~~~~~~~~~~~~~~~~~~ \underset{0 \leq j \text{\lt} n-1}{\bigwedge}[\underset{0 \leq l \text{\lt} |w|}{\bigwedge}  i_j = l \implies p_{j} = w(l)]\\
     ~~~~~~~~~~~~~~~~~~~ \underset{0 \leq j \text{\lt} n-2}{\bigwedge}[\underset{0 \leq l \text{\lt} |w|}{\bigwedge}  \varphi_{trend}(i_j,i_{j+1},l)]
\end{array}
\]
}}




==> intro-suffix.tex <==

We next present the components of our approach:
\begin{inparaenum}[(i)]
  \item the mathematical representation for defining charts precisely,
  \item the process for learning the mathematical representation, and
  \item the process for synthesizing pattern queries.
\end{inparaenum}
\subsubsection{Chart Representation (Sections \ref{Se:overview:problemdef}, \ref{Se:newformal})}
We represent charts as conjunctions of constraints pertaining to the relative comparison between price pairs.
For example, the head and shoulders pattern is captured by the formula:
\vspace{-0.21cm}
\[
\begin{array}{l}
\varphi_{HS}(p_0,...,p_6) =
%\ltpred{p_0}{p_1} \land \ltpred{p_2}{p_1} \land \ltpred{p_1}{p_3} \land \ltpred{p_5}{p_3} \land \\
%~~~~~~ ~~~~~~~~~~~~\ltpred{p_4}{p_5} \land \ltpred{p_6}{p_5} \land \ltpred{p_0}{p_2} \land \ltpred{p_2}{p_4} \land \ltpred{p_0}{p_6}
\ltpred{p_0}{p_2} \land \ltpred{p_2}{p_1} \land \ltpred{p_1}{p_3} \land \ltpred{p_2}{p_4} \land \\
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\ltpred{p_4}{p_5} \land \ltpred{p_5}{p_3} \land \ltpred{p_6}{p_0}
\end{array}\vspace{-0.21cm}
\]
where $p_0,...,p_6$ are prices in a time point series, $p_0$ is the price at the earliest time point, and $p_6$ is the price at the latest.
%In~\secref{overview:learning}, we explain how to learn this formula.

A major challenge is how to obtain such mathematical description from visual patterns, as
\href{http://www.metastock.com/customer/support/kb/faq.aspx?fc=96}{MetaStock's FAQ} explains:
\begin{myquote}
  \emph{Chart patterns are visual and very subjective, which means they cannot usually be broken down to mathematical terms. If you can explain the patterns mathematically to MetaStock, it will be able % to plot a formula
  to identify when the mathematical conditions occur in a chart.% If you cannot [...] %discover a way to
%  explain the patterns mathematically to MetaStock it will not be possible [...].%to write formula for the patterns.
  }
\end{myquote}\vspace{-0.2cm}
Namely, learning a formula is a stepping stone towards writing queries. Further, formulas act as an intermediate representation which separate the learning phase from the code generation phase and allows {\tool} to synthesize different implementations, potentially for different trading platforms.

\subsubsection{The Formula Learning Process (Sections \ref{Se:overview:learning}, \ref{Se:algo})}
To learn a formula, {\tool} examines all potential constraints. %, which are the constraints satisfied by the example chart.
For each constraint, {\tool} generates a chart and asks the user
to determine whether this chart is indicative of the pattern. Accordingly, {\tool} infers whether this constraint should appear in the formula.
Generating charts is not trivial and to the best of our knowledge, we are the first to show how to systematically generate charts for learning chart patterns.

\begin{comment}
For each constraint, {\tool} generates a special chart \emph{not} satisfying it, and asks the user
to provide binary feedback on whether this chart is indicative of the pattern. If not, the constraint will appear in the formula.
Otherwise, it will not appear.


\begin{figure}
\centering
  \adjustbox{valign=t}{\includegraphics[height=3cm,width=8.3cm,clip=true, trim = 0pt 1pt 0pt
  0pt]{figures/intro_figs.png}}
  \caption{Learning a Formula from One Chart.}
  \figlabel{flowIntro}
\end{figure}

\begin{Example}\exlabel{Ex1}
Consider an initial chart example (\figref{flowIntro}(a)) for learning
the head and shoulders pattern. Eventually, {\tool} will learn the formula $\varphi_{HS}$.
To learn $\varphi_{HS}$, {\tool} examines every relationship between pairs of points satisfied
by the example, among them $p_4$$\prec$$p_1$ and $p_5$$\prec$$p_3$. The chart for examining
$p_4$$\prec$$p_1$ (\figref{flowIntro}(b)) is accepted by the user and thus $p_4$$\prec$$p_1$ will not appear in $\varphi_{HS}$, whereas
the chart for examining $p_5$$\prec$$p_3$ (\figref{flowIntro}(c)) is not accepted and thus $p_5$$\prec$$p_3$ will appear in $\varphi_{HS}$.
%For each constraint, {\tool} generates a chart \emph{not} satisfying it ().
% The analyst is required to provide a binary feedback on whether this chart is indicative of the pattern.
%In this example, the two relevant points are emphasized in red rectangles. %(the analyst does not see red points, we simply use red for illustration purposes).
%Based on the yes or no feedback, the synthesizer learns whether $p_4<p_1$ appears in the pattern formula.
\end{Example}
\end{comment}

%By communicating only through charts, {\tool} relieves analysts from the need to understand logical constraints.
\spara{Generating Charts}
To generate a chart, {\tool} searches for an assignment satisfying a special set of constraints using an SMT solver. The chart is then generated from the assignment.
A challenge arises if this set of constraints is not satisfiable, in which case {\tool} relaxes it carefully and generates the chart from an assignment satisfying the relaxed set.

%The minimal number is crucial for correctness (\appref{correctness}).

\ignore{
\para{Advantages of Declarative Queries}
Representing patterns via declarative queries (i.e. logical formulas) has several advantages. First, formulas are a natural way to describe constraints. For instance, consider the head and shoulders pattern captured by the formula:
\vspace{-0.15cm}
\[
\begin{array}{l}
\varphi_{HS}(p_0,...,p_6) =
%\ltpred{p_0}{p_1} \land \ltpred{p_2}{p_1} \land \ltpred{p_1}{p_3} \land \ltpred{p_5}{p_3} \land \\
%~~~~~~ ~~~~~~~~~~~~\ltpred{p_4}{p_5} \land \ltpred{p_6}{p_5} \land \ltpred{p_0}{p_2} \land \ltpred{p_2}{p_4} \land \ltpred{p_0}{p_6}
\ltpred{p_0}{p_2} \land \ltpred{p_2}{p_1} \land \ltpred{p_1}{p_3} \land \ltpred{p_2}{p_4} \land \\
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\ltpred{p_4}{p_5} \land \ltpred{p_6}{p_5} \land \ltpred{p_5}{p_3} \land \ltpred{p_6}{p_0}
\end{array}\vspace{-0.15cm}
\]
where $p_0,...,p_6$ are the stock prices in a time point series, $p_0$ is the price at the earliest time point, and $p_6$ is the price at the most recent time point. This declarative representation is shorter than the one in~\figref{streaminsight} and clearer than any procedural code. Second, formula representation allows to easily detect charts which are \emph{close to the pattern} (e.g., violate one or two constraints), a step that may be beneficial to analysts. Third, formulas abstract away noise. For example, using $\varphi_{HS}$, {\tool} would detect the pattern occurrence in \figref{HeadShoulders}, whereas the state machine of \figref{streaminsight} would miss it.
}

%{\tool} provides the user the ability to focus on confined-segments of the stream and classify them manually.
%Then,
%{\tool} will search how to apply a minimal number of updates to the formula
%to capture the desired behaviour. Furthermore, {\tool} allows the user to
%mark which points construct the pattern, in case a positive occurrence was
%missed by the formula.

\spara{Formula Update}
{\tool} enables analysts to update formulas. % if they find their definition of the pattern too strict or permissive.
The update is accomplished by presenting new chart examples to {\tool}, which in turn looks for the minimal changes to the formula required to adapt to the new examples.
\ignore{\para{Reporting on Similar Occurrences}
{\tool} can be adjusted to present the user occurrences violating at most $k$ constraints, where $k$ is a parameter determined by the user. This may assist the analysts to update their formula if they are not sure about the pattern constraints.}



\subsubsection{The Synthesis Process (Sections \ref{Se:overview:synthesis}, \ref{Se:amibroker})}
Given a formula, {\tool} synthesizes a query in AFL, AmiBroker's DSL. For example, {\tool} synthesized the query in \figref{code-headns} from $\varphi_{HS}$.
While AmiBroker is one of the fastest trading platforms, it requires expertise for writing correct and efficient queries, as the AFL manual warns:
%
\begin{myquote}
  \emph{Poor formula coding is the foremost reason of slow down. People coming from
``other'' languages often do not realize the full potential of AFL array processing
and code everything ``old'' style (i.e. with loops). %Loops can be 10..50 times slower than equivalent array-based code.
}
\end{myquote}
%
Thus, synthesized code may be more efficient than hand-crafted code written by non-experts. The key challenge in synthesizing the query is in generating the code that selects the price points from the stream. This is evident in \figref{code-headns} -- all lines except the last are used for defining the price points.
%{\tool} synthesizes array-based code from formulas. Translating the formula (after {\tool} learned it) may be simple,
%but generating the code that picks the price points from the stream is more subtle. This is evident in
%\figref{code-headns}, %which shows the code from a formula capturing the head and shoulders -- only the last line describes the formula.
%which shows the code synthesized from $\varphi_{HS}$ -- only the last line describes the formula.


==> mainalgo.tex <==
\begin{algorithm}[t]
\small
\dontprintsemicolon
\linesnumbered
\SetLine
\restylealgo{boxed}
examplePattern = getPattern(example) \; \lnlabel{examplePattern}
processedData = analyzeWindows(windows, examplePattern)\; \lnlabel{analyzeWindows}
graph = constructGraph(examplePattern, processedData)\; \lnlabel{graph}
queue = sortNodes(graph) \; \lnlabel{queue}
\While{classification is not done}{ \lnlabel{LoopBegin}
    node = queue.pop()\; \lnlabel{pop}
    response = consultUser(node) \; \lnlabel{consult}
    deduce(node, response, graph, queue) \; \lnlabel{deduce}
}\lnlabel{LoopEnd}
\caption{\toolname(example, windows)}\label{Alg:MainAlg}
\end{algorithm}


==> overview2_-_Copy.tex <==
\section{Overview}\seclabel{Overview}
In this section, we informally explain \name\ and \alg.


\input{gridfigure}
\subsection{Exact Learning from Examples}\seclabel{overview1}
We address the problem of exact learning from examples (\name). In \name, the user provides some initial positive and negative examples, and the goal is to learn the \emph{concept} the user wishes to capture. A concept is a subset of the example domain, every example in the concept is a \emph{positive example} and every other example is a \emph{negative example}. That is, it includes all the positive examples and none of the negative ones.
For example, consider the domain, $D=\{(x,y)\mid~0\leq x \leq 4,0 \leq y \leq 4\}$, and assume a user wishes to learn the concept $\{(1,1),(1,2),(2,1),(2,2)\}$ and provides a single
positive example, $(2,2)$. \figref{Simple} shows the domain where the concept is marked with green, bold points.

\para{The Challenge of Exact Learning}
Exact learning algorithms have to learn the single concept, however the initial examples the user provides are often consistent with many concepts. To illustrate, in our example, there are many subsets of $D$ that contain the positive example $(2,2)$.
To isolate the correct concept, exact learning algorithms are allowed to present questions to the user. This enables to prune the space of concepts consistent with the examples until only a single concept remains.

\para{Membership Queries} Two common questions presented by exact learning algorithms are \emph{membership queries} and \emph{validation queries}.
Membership queries present examples and ask whether they belong to the concept, while validation queries present concepts and ask whether these are the correct concepts. Unfortunately, in many domains, validations queries are complex, error-prone, or impossible for the user to understand. For such domains, it is desirable to limit the questions to membership queries only, namely limit the setting to \name: exact learning from examples.

\para{Predicate-defined Concepts}
Often, concepts are not defined directly as any subset of the domain, but rather using \emph{features} or properties of the concepts. %Though, the features sometimes may restrict the concept space, typically these do not impose a real restriction.
In this work, we assume a general setting of \name\ where concepts are defined using arbitrary predicates.
For example, consider our running example, and assume that the concepts are expressed using the set of predicates
$S=P_x \cup P_y \cup \{x=y\}$, where $P_x$ consists of all predicates capturing intervals of $x$:
 \[
\begin{array}{lll}
P_x &=& \{\rangep{x}{0}{2}, \rangep{x}{1}{3}, \rangep{x}{2}{4}\}
%P_x &=& \{(0 \leq x \leq 2), (0 \leq x \leq 3), \dots, (0 \leq x \leq 1000), \\
%&& (1 \leq x \leq 3),  (1 \leq x \leq 4), \dots, (1 \leq x \leq 1000),\\
%&&    ... \\
% &&   (998 \leq x \leq 1000)\}=\{ i \leq x \leq (1000 - j) \mid \\
%&&i < (999 - j) \land 0 \leq i \leq 1000, 0 \leq j \leq 1000 \}
\end{array}
\]
$P_y$ is defined identically with respect to $y$. A concept satisfies the predicate $a \leq x \leq b$ if all its points $(x,y)$ satisfy that $x$ is between $a$ and $b$, and a concept satisfies the predicate $x=y$ if all its points take the form $(x,x)$.
Using these predicates, the concept we wish to learn is: $$(1\leq x \leq 3) \land (2 \leq x \leq 4) \land (1\leq  y\leq 3) \land (2 \leq y \leq 4)$$

%\emph{Thereby, we can design a synthesis algorithm that interacts with the user only through examples, yet can guarantee that the learned concept captures precisely the user intent.}
%This general setting introduces new challenges and thus cannot be solved using existing techniques for exact learning,

\para{Finding the Correct Concept} To learn the concept formula, one has to present examples to the user and prune the inconsistent concepts, until a single concept remains.
Classical exact learning algorithms may be used only if the predicates are independent. Unfortunately, domains relevant for program synthesis often define specifications over abstract properties that may be dependent.
A different approach~\cite{BitManipulation:2010} that does address this challenge iteratively picks two non-equivalent concepts, shows an input distinguishing them, asks the user for the correct output, and accordingly prunes the inconsistent concepts. Unfortunately, since the two concepts are picked arbitrarily, the number of concepts pruned after a single question may be small, which may result in presenting an exponential number of questions even when a linear number suffices (see~\secref{eval}).
In contrast, we leverage the partial-order between the concepts to pick two ``close'' concepts at each step, and this guarantees that overall a minimal number of questions is presented.

In the rest of the section, we focus on learning conjunctions over a set of predicates $S$. We later show that learning disjunctions is dual, and these techniques can be used to learn CNFs and DNFs.

\begin{figure*}
\centering
  \includegraphics[page=2,height=5cm,width=17cm,clip=true,trim=0pt 20pt 0pt 0pt]{figures/concept_space}
  \caption{The partially-ordered concept space that \alg\ traverses along and distinguishing inputs showed by \alg.}
  \figlabel{conspace}
\end{figure*}



\subsection{Our Approach: a Guided Traversal in the Concept Space}\seclabel{congraph}
wwwOur approach hinges on two main ideas:
\begin{inparaenum}[(i)]
\item we use the structure of the formula to pick the next question to be presented to the user
\item when the question cannot be directly presented to the user, we leverage a partial order between concepts to define the minimal set of questions that can be presented to the user, and when classified provide an answer for the original question.
\end{inparaenum}

Conceptually, \alg\ traverses along the \emph{partially-ordered} space of concepts consistent with the examples to find the correct concept formula $\varphi_C$. The partial-order is defined as follows: two formulas $\varphi,\psi$ satisfy $\varphi \leq \psi$ if $\varphi$ contains all of $\psi$'s predicates (and possibly additional predicates). This order induces a graph of the concepts consistent with the observed examples: the nodes are the consistent concepts, captured by formulas, and there is an edge between two formulas $\varphi$ and $\psi$ if there is no other formula $\psi'$ satisfying $\varphi \leq \psi' \leq \psi$. This space is known as the version space~\cite{Mitchell82}.
\figref{conspace} presents part of this graph corresponding to our running example: the bottom most node shows the most specific concept formula, $\varphi_0$, which satisfies all predicates from $S$ satisfied by the initial positive example $(2,2)$. Edges link $\varphi_0$ to more relaxed formulas, namely formulas with fewer constraints. We denoted by $\varphi_0^{R_1,...,R_n}$ the formula $\varphi_0$ without the predicates $R_1,...,R_n$.

To learn the concept formula, one has to present examples to the user and prune the inconsistent nodes, until a single node remains. We present \alg, a guided traversal that at each step examines a certain node %(the first is the most strict concept consistent with the initial examples)
and examines its immediate neighbours to find a direct path to the concept formula.
An immediate neighbour of a node $\varphi$ is $\varphi^R$, which is identical to $\varphi$ except for a single predicate $R$ which is dropped. Examining this neighbour means to check whether $\varphi_C$ is reachable from it, i.e., whether $R$ is in $\varphi_C$.

To check if $R$ is part of $\varphi_C$, \alg\ looks for a distinguishing input between $\varphi$ and $\varphi^{R}$.
Since $\varphi$ implies $\varphi^R$, this means to find an example satisfying $\varphi^R \wedge \neg \varphi$.
If there is such an example, its classification enables to progress: if this is a positive example (i.e., it satisfies $\varphi_C$), \alg\ proceeds towards $\varphi^R$ (and prunes the rest of the space), and otherwise, $\varphi_R$'s sub-graph is pruned. In the special case where predicates are independent, namely for every choice of literals over these predicates there is a satisfying example,
it is guaranteed that such distinguishing inputs always exist, and thus every predicate can be classified with a single question. In fact, this is a classical exact learning algorithm for domains having this property. However, we address the general case, where predicates may be dependant, and thus we address a novel challenge of how to obtain alternative distinguishing inputs that enable to classify $R$.

A na\"ive solution to this challenge is to examine every child of $\varphi^R$: if all have distinguishing inputs with $\varphi$ and one of these inputs is a positive example (satisfies $\varphi_C$), the traversal proceeds towards this child and prunes the rest of the space; otherwise, if all inputs are negative examples, $\varphi^R$'s sub-graph is pruned. However, it is not guaranteed that the children necessarily have distinguishing inputs, in which case \emph{their} children must be examined similarly. While this solution is correct, it is very expensive in the number of questions. This leads us to the second challenge we address: how to obtain \emph{a minimal number} of alternative distinguishing inputs.

To present a minimal number of questions, we show that instead of examining all children of $\varphi_R$, it suffices to examine a certain \emph{subset} of them. This subset is the set of predicates in $\varphi_R$ ``preventing''
distinguishing inputs with $\varphi$, namely predicates preventing the formula $\varphi_R \wedge \neg \varphi$ from being satisfiable. Such predicates are known as \emph{the unsat core} of the formula. Namely, we prove that if there is no distinguishing input for $\varphi_R$ and $\varphi$, it suffices to compute an unsat core of the above formula and consider only the children belonging to the unsat core. If the computed unsat cores are guaranteed to be minimal, we prove that a minimal number of questions is presented.
Though finding minimal unsat cores in general theories is an EXPSPACE-complete, there are approaches to compute small unsat cores (e.g.,~\cite{CimattiGS11}), and in some theories (such as the ones exemplified in this work), minimal unsat cores can be computed.

%To guarantee the minimal number of questions, \alg\ generates a minimal number of examples to classify each predicate.
%In the best case, if the predicates are independent, each can be classified using a single example (in fact, only such domains were addressed by former \name\ algorithms). However, in the general case predicates may be dependant, in which case, more examples may be needed. We next demonstrate this process on our running example.



%However, if when examining $\varphi^R$ there is no distinguishing input, then to make progress, \alg\ considers the unsat core of $\varphi_R$, which determines which children of $\varphi^R$ should be examined to decide whether to proceed in this sub-graph or prune it. If one of these children corresponds to a positive example, then \alg\ can continue towards this node (and prune the rest of the space).
%However, if all the corresponding examples are negative, then \alg\ can only infer that $\varphi_C$ is not reachable through the sub-graph of $\varphi^R$, namely $R$ is part of $\varphi_C$ and thus \alg\ continues towards a different node directly connected to $\varphi$. This view demonstrates the need in minimal cores: if a core is not minimal, more children are examined before \alg\ safely prunes $\varphi^R$'s sub-graph. We note that if one of $\varphi^R$'s children, $\varphi^{R,R'}$, also does not have a distinguishing input, then an additional unsat core is computed, and $\varphi^{R,R'}$'s classification is determined by its children.

%We next describe \alg's guided traversal and exemplify on our running example.
% We focus on the case of learning conjunctions over a set of predicates $S$. We later show that learning disjunctions is dual, and these techniques can be used to learn CNFs and DNFs.


%First, \alg\ computes the most strict concept formula $\varphi_0$ which is the conjunction $\bigwedge_{l \in S_0} l$ where $S_0$ is the set of predicates from $S$ satisfied by the initial positive examples. In our example, $(2,2)$ is the single initial positive example and thus:
%\[
%\begin{array}{lll}
%\varphi_0 & = & \rangep{x}{0}{2} \land \rangep{x}{1}{3} \land\rangep{x}{2}{4}\land \\
%&&\rangep{y}{0}{2} \land\rangep{y}{1}{3} \land\rangep{y}{2}{4} \land (x = y)
%\end{array}
%\]
 %Then, \alg\ attempts to classify the predicates and begins with $\rangep{x}{0}{2}$. However, $\varphi_0^{\rangep{x}{0}{2}}$ has no distinguishing input with $\varphi_0$ (denoted by a dashed circle at \figref{conspace}), and thus \alg\ computes an unsat core, which determines which children of $\varphi_0^{\rangep{x}{0}{2}}$ should be examined. In our example, these are $\varphi_0^{\rangep{x}{0}{2},x=y}$ and $\varphi_0^{\rangep{x}{0}{2},\rangep{y}{0}{2}}$. Both have distinguishing examples, which are classified as negative, and thus enable \alg\ to entirely prune $\varphi_0^{\rangep{x}{0}{2}}$'s sub-graph and proceed towards a different node. The next step of \alg\ is to examine the node $\varphi_0^{\rangep{x}{2}{4}}$, which also does not have a distinguishing input. After obtaining the unsat core, \alg\ examines the nodes $\varphi_0^{\rangep{x}{2}{4},x=y}$ and $\varphi_0^{\rangep{x}{2}{4},\rangep{y}{2}{4}}$, which both have distinguishing inputs: $(1,2)$ and $(1,1)$. After presenting the first example to the user, and discovering it is a positive example, \alg\ discards the second example, and proceeds toward the node $\varphi_0^{\rangep{x}{2}{4},x=y}$, essentially pruning the rest of the space.

%Many algorithms traverse this space, however \alg\ is the first to provide a \emph{guided} traversal, using only examples, and without assuming that predicates are independent. A close work to \alg\ is the \emph{oracle-based synthesis}~\cite{BitManipulation:2010}, which implements an unguided traversal in this space: at each step, it looks for two nodes with a distinguishing input, and based on the input's output, some nodes are pruned (all the nodes inconsistent with the output).


\subsection{A Running Example}
In this section, we exemplify \alg\ on the concept defined in~\secref{overview1}.
Given the initial example the user provides, $(2,2)$, \alg\ first computes the most strict concept consistent, $\varphi_0$ (i.e., it implies every consistent concept), which is $\bigwedge_{l \in S_0=\{(2,2) \models R \mid R\in S\}} l$, i.e.,:
\[
\begin{array}{lll}
\varphi_0 & = & \rangep{x}{0}{2} \land \rangep{x}{1}{3} \land\rangep{x}{2}{4}\land \\
&&\rangep{y}{0}{2} \land\rangep{y}{1}{3} \land\rangep{y}{2}{4} \land (x = y)
\end{array}
\]


%\para{Learning the Correct Concept} To learn the formula capturing the correct concept, $\varphi_C$, \alg\ examines each predicate and checks which is part of $\varphi_C$. To this end, for each predicate $R$ in $\varphi_0$ \alg\ generates examples, presents to the user, which classifies them as belong to the concept or not, and accordingly infers whether $R$ is in $\varphi_C$.

\para{Distinguishing Inputs} After constructing $\varphi_0$, \alg\ looks for a predicate $R$ that can be classified with a
single example. Unfortunately, none of its immediate neighbours in the concept graph has a distinguishing inputs with $\varphi_0$. For example, for
  $R=\rangep{x}{0}{2}$ there is no distinguishing input, because such an input has to satisfy the (unsatisfiable) formula, $\varphi_0^R \wedge \neg \varphi_0$, which is simplified to:

\[
\begin{array}{ll}
\psi_{S_0}^{\rangep{x}{0}{2}}&\hspace{-0.3cm}\triangleq \bigwedge_{l \in S_0 \setminus \{\rangep{x}{0}{2}\}} l \land \neg \rangep{x}{0}{2} =\\
&\hspace{-0.3cm}\neg \rangep{x}{0}{2} \land \rangep{x}{1}{3} \land \rangep{x}{2}{4}\land \\
&\hspace{-0.3cm}\rangep{y}{0}{2} \land \rangep{y}{1}{3} \land\rangep{y}{2}{4} \land (x = y)
\end{array}
\]

This formula is unsatisfiable due to the dependency between the predicates, $\rangep{x}{0}{2}$, $\rangep{y}{0}{2}$, and $x=y$: there are no examples satisfying that $x$ is greater than $2$, $y$ is at most $2$, and $x$ equals $y$. Thus, there is no distinguishing input as required.


% and thus it looks for a predicate requiring a minimal number of examples. As we shortly explain, $\rangep{x}{0}{2}$ is one of these predicates. Ideally, $\rangep{x}{0}{2}$  can be classified with a single example. This is the case if there is a \emph{distinguishing input} between the formula $\varphi_0$ and the formula identical to $\varphi_0$ but with $\rangep{x}{0}{2}$ dropped, denoted by $\varphi_0^{\rangep{x}{0}{2}}$.
%Since $\varphi_0$ implies ${\varphi_0}^{\rangep{x}{0}{2}}$, a distinguishing input is an assignment to ${\varphi_0^{\rangep{x}{0}{2}}}$ not satisfying $\varphi_0$. Such an input enables to classify $\rangep{x}{0}{2}$:
%if the user classifies this input as a positive example, namely, there are two positive examples that satisfy the same constraints only that one satisfies $\rangep{x}{0}{2}$ and the other does not, then $\rangep{x}{0}{2}$ is not part of $\varphi_C$;
 % otherwise, $\rangep{x}{0}{2}$ must be part of $\varphi_C$.

%\para{Constructing Distinguishing Inputs} A distinguishing input to $\varphi_0$ and $\varphi_0^{\rangep{x}{0}{2}}$ is \emph{any} assignment to the formula ${\psi}^{\rangep{x}{0}{2}}_{S_0}$, which is identical to $\varphi_0$
%except for $\rangep{x}{0}{2}$ that is negated, that is:

%\[
%\begin{array}{ll}
%\psi_{S_0}^{\rangep{x}{0}{2}} &=\neg \rangep{x}{0}{2} \land \rangep{x}{1}{3} \land \\
%&\phantom{=}\rangep{x}{2}{4}\land \rangep{y}{0}{2} \land\\
%&\phantom{=}\rangep{y}{1}{3} \land\rangep{y}{2}{4} \land (x = y)
%\end{array}
%\]

%Unfortunately, this formula is unsatisfiable. This is due to the dependency between the predicates, $\rangep{x}{0}{2}$, $\rangep{y}{0}{2}$, and $x=y$: there are no examples satisfying that $x$ is greater than $2$, $y$ is at most $2$, and $x$ equals $y$. Thus, there is no distinguishing input as required.

%\para{The Challenges of Dependencies in \name} The former scenario exemplifies the motivation for addressing the two challenges of learning formulas over dependent predicates:
%\begin{inparaenum}[(i)]
%  \item how to construct alternative satisfiable formulas that their examples can be used to classify the predicate at hand (in our example, $\rangep{x}{0}{2}$), and
%  \item how to present a minimal number of questions to the user.
%\end{inparaenum}

\para{Finding Alternative Distinguishing Inputs}
To find alternative satisfiable formulas, \alg\ computes an \emph{unsat core} of the above formula. For each predicate $R'$ in the unsat core (except for the one at hand, $R$), \alg\ constructs a formula that negates $R'$, in addition to $R$.
If some of these formulas are still unsatisfiable, \alg\ repeats this process, namely computes a (new) unsat core, and generates a set of formulas from it.
Finally, \alg\ presents the user an example for each of these formulas.
In our example, \alg\ computes an unsat core of ${\psi}_{S_0}^{\rangep{x}{0}{2}}$, which is $\{\rangep{x}{0}{2},\rangep{y}{0}{2},x=y\}$ and generates the formulas
${\psi}_{S_0}^{\rangep{x}{0}{2}, (x=y)}, {\psi}_{S_0}^{\rangep{x}{0}{2}, \rangep{y}{0}{2}}$. These formulas are satisfiable, by $(3,2)$ and $(3,3)$ respectively, and thus \alg\ presents these points to the user.

\para{Inferring Classifications from the Alternative Formulas}
If one of these examples, corresponding to $\psi^{R,R_1,...,R_k}_{S_0}$, is classified by the user as a positive example, then none of the negated predicates is part of $\varphi_C$, and thus $R,R_1,...,R_k$ are dropped from the current formula. However, if all of them are negative, then it is only guaranteed that the predicate at hand, $R$, is part of the correct concept $\varphi_C$.
For example, in our example, both points $(3,3)$ and $(3, 2)$ are negative, and thus \alg\ infers that $\rangep{x}{0}{2}$ is part of $\varphi_C$. Note that though these formulas negate additional predicates, $x=y$ and $\rangep{y}{0}{2}$, these cannot be classified at this point. Indeed, eventually $x=y$ will be dropped, while $\rangep{y}{0}{2}$ will be part of $\varphi_C$.
However, the next step of \alg, that considers the predicate $\rangep{x}{2}{4}$, infers differently. Similarly to before, there is no distinguishing input for $\varphi_0$ and $\varphi_0^{\rangep{x}{2}{4}}$ (i.e., ${\psi}^{\rangep{x}{2}{4}}_{S_0}$ is unsatisfiable), and thus \alg\ considers the unsat core $\{\rangep{x}{2}{4},\rangep{y}{2}{4},x=y\}$ and generates the relaxed formulas ${\psi}_{S_0}^{\rangep{x}{2}{4},x=y}$ and ${\psi}_{S_0}^{\rangep{x}{2}{4},\rangep{y}{2}{4}}$. Both formulas are satisfiable, by $(1,2)$ and $(1,1)$, and both are positive. However, this time after the first example, $(1,2)$, is presented to the user, \alg\ infers immediately (without presenting $(1,1)$) that $\rangep{x}{2}{4}$ \emph{and} $x=y$ are not in $\varphi_C$, and thus it updates the current candidate formula to $\varphi_0^{\rangep{x}{2}{4},x=y}$.
In the next step, \alg\ looks for distinguishing inputs from the new candidate formula, and so it constructs $\psi_{S_0 \setminus \{{\rangep{x}{2}{4},x=y}\}}^{\rangep{y}{2}{4}}$, namely it ignores the predicates $\rangep{x}{2}{4},x=y$, as they no longer affect the classifications.
%Note that $(1,1)$ will be used in the next step to classify $\rangep{y}{2}{4}$, as it is the distinguishing input for $\varphi_0^{\rangep{x}{2}{4},x=y}$ and $\varphi_0^{\rangep{x}{2}{4},x=y,\rangep{y}{2}{4}}$.
We note that in fact $\rangep{x}{2}{4}$ is implied by the predicate $\rangep{x}{0}{2}$, and thus is classified as redundant by \alg\ immediately after learning $\rangep{x}{0}{2}$, we ignore this step here to exemplify how \alg\ classifies a predicate as not part of $\varphi_C$.
%\para{Removing Implied Predicates} After classifying a predicate as part of the formula $\varphi_C$, it may be the case that some predicates are implied and thus need not be classified further. For example, in our example after classifying $\rangep{x}{0}{2}$ as part of $\varphi_C$, the predicate $\rangep{x}{2}{4}$ is implied and thus classified immediately.

%\para{Presenting a Minimal Number of Questions} We prove that \alg\ presents a minimal number of questions, assuming that the unsat cores computed are minimal. Though finding minimal unsat cores in general theories is an EXPSPACE-complete, there are approaches to compute small unsat cores (e.g.,~\cite{CimattiGS11}), and practically on some theories (such as the ones we exemplify in this work), current SMT-solvers, e.g., Z3~\cite{DeMoura:2008} can compute minimal unsat cores.

% Thus, \alg\ can update the current hypothesis to $\varphi_0^{\rangep{x}{0}{2}}$.

%To check whether $\rangep{x}{0}{2}$ can be dropped, \alg\ wishes to construct a \emph{distinguishing example} between the current hypothesis $\varphi_0$ and $\varphi_0$ without $\rangep{x}{0}{2}$, which we denote by .
%, the algorithm constructs a formula where the predicate is negated and attempts to find a concrete example that can be presented to the user for classification. For example, we check whether the predicate $\rangep{x}{0}{2}$ can be dropped,  by constructing the formula $\widetilde{\varphi_{1}}$ where $\rangep{x}{0}{2}$ is negated:


%Using the shorthand defined earlier, we can write this formula as:
%\[
%\widetilde{\varphi_1} = \varphi_0 \setminus \{ \rangep{x}{0}{2} \}
%\]




\subsection{\alg\ Extensions}
We use the logic described for learning formulas over conjunctions, to learn other concept classes: disjunctions, CNFs and DNFs.

\para{D-\alg} The disjunctive variation of \alg\ is dual to the conjunctive.
While the conjunctive variation, C-\alg, generalizes from the positive examples, and learns which constraints must be met by examples in the concept, D-\alg\ generalizes from the \emph{negative} examples, and learns which constraints eliminate examples from being part of the concept.
\figref{conspace2} visually demonstrates the difference between the classes:
C-\alg\ learns a consecutive region in the concept space that contains all positive examples, while D-\alg\ learns the same region only for the negative examples.

\para{The General \alg} The general \alg\ algorithm learns CNFs and DNFs, namely concepts in which the negative examples (in CNFs) or positive examples (in DNFs) are not necessarily in a single consecutive region. If the user could guarantee that she provided a representative of each region, \alg\ could have simply invoke D-\alg\ to learn a CNF (or C-\alg\ to learn a DNF) \emph{separately} on each example and unite the set of clauses (or cubes) to a conjunction (or disjunction). However, \alg\ does not assume this, and thus has to actively:
\begin{inparaenum}[(i)]
  \item determine when it is missing a representative, and
\item obtain a concrete representative from a missing region.
\end{inparaenum}
We leverage the fact that every formula can be represented both as a CNF and a DNF to address both challenges with a single check: \alg\ simultaneously learns both a CNF (from the negative examples) \emph{and} a DNF (from the positive examples) and terminates only when these are equivalent, in which case it is guaranteed that all regions are covered. As long as the formulas are not equivalent, \alg\ automatically finds an example classified differently by the formulas (namely, it is from a missing region), asks for its output, accordingly tightens either the CNF or the DNF, and checks again whether now the two formulas are equivalent.


\begin{figure}
\centering
  \includegraphics[page=1,height=4.5cm,width=7cm,clip=true,trim=0pt 0pt 600pt 0pt]{figures/overview_2}
  \caption{Illustration of the concept spaces.}
  \figlabel{conspace2}
\end{figure} 

==> results-pattern.tex <==
%\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
%\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\begin{table}\centering
%\begin{wrapfigure}[22]{r}{0.54\textwidth}\vspace{-0.cm}\hspace{-0.25cm}
\scriptsize
\ra{1.2}
\begin{tabular}{p{1.cm}p{0.22cm}p{0.22cm}p{0.22cm}p{0.5cm}p{0.22cm}p{0.5cm}p{0.22cm}p{0.22cm}p{0.22cm}p{0.22cm}}
\toprule
     &  & & & \multicolumn{2}{c}{C-\alg} & \multicolumn{4}{c}{Oracle-Based \cite{BitManipulation:2010}} &\\
Pattern & $|S_{0}|$ & Def. & $|S_{P}|$ & time & \#Q & time & Avg. & Max & Min\\
\midrule
\multirow{5}{1.2cm}{Head and Shoulders} &\multirow{5}{0.5cm}{42}& \ref{head2}  &6& 360 & 18 & 139 & 44.4 & 57 & 38 & \\
&&\ref{head3} &10  & 223 & 18 & 142 & 54.8 & 61 & 43 & \\
&& \ref{head4}&10& 344 & 17 & 155 & 61.1 & 88 & 43 & \\
&& \ref{head5}&7& 285 & 14 & 132 & 50.6 & 71 & 40 & \\
&& \ref{head1}&6& 267 & 12 & 147 & 58.4 & 77 & 37 & \\ \midrule
%\multirow{5}{1.2cm}{Cup and Handle} &~~~~\multirow{5}{0.5cm}{8}&\multirow{5}{0.5cm}{56}& \ref{cup1}& 9& 45 &0.286 {\scriptsize(0.143)} & 0.509\\
%&&&\ref{head3} &56 &11&23\\
%&&&\ref{cup2}&10&34&0.085 {\scriptsize(0.062)} & 0.193\\
%&&& \ref{cup3}&11&25&0.082 {\scriptsize(0.066)} & 0.2\\
%&&& \ref{cup4}&11&24& 0.084 {\scriptsize(0.067)} & 0.219\\
%&&& \ref{cup5}&9&9&0.286 {\scriptsize(0.143)} & 0.509\\\midrule
\multirow{5}{1.2cm}{Cup with Handle} &\multirow{5}{0.5cm}{30}& \ref{cup1}& 5& 107 & 12 & 82 & 38.3 & 48 & 27 & \\
&&\ref{cup2}&6& 93 & 12 & 82 & 43.6 & 57 & 33 & \\
&& \ref{cup3}&7 & 232 & 13 & 70 & 35.1 & 41 & 28 & \\
%&& \ref{cup4}&11&24& 0.084 {\scriptsize(0.067)} & 0.219\\
&& \ref{cup4}& 7 & 184 & 13 & 66 & 36.4 & 41 & 32 & \\
&& \ref{cup5}&5 & 111 & 10 & 69 & 38.6 & 45 & 22 & \\\midrule
\multirow{4}{1.2cm}{Two Tops} &\multirow{4}{0.5cm}{20}& \ref{top1}& 6 & 56 & 9 & 29 & 19.4 & 20 & 18 & \\
&&\ref{top2}&6 & 49 & 9 & 29 & 18.3 & 20 & 16 & \\
&& \ref{top3}&6 & 56 & 7 & 28 & 18.7 & 19 & 17 & \\
&& \ref{top4}&4 & 56 & 6 & 25 & 17.0 & 17 & 17 & \\ \midrule
\multirow{2}{1.2cm}{Symmetrical Triangle} &\multirow{2}{0.5cm}{42}& \ref{trian1}&7 & 23 & 16 & 186 & 71.4 & 76 & 62 & \\
&& \ref{trian2}& 7 & 239 & 14 & 165 & 66.5 & 78 & 37 & \\ \midrule
\multirow{2}{1.2cm}{Flag} &\multirow{2}{0.5cm}{42}& \ref{flag1}&7 & 706 & 17 & 175 & 64.0 & 89 & 52 &\\
&& \ref{flag2}& 6 & 67 & 16 & 136 & 54.3 & 90 & 43 &\\\midrule

\multirow{2}{1.2cm}{Rectangle} &\multirow{2}{0.5cm}{20}& \ref{rec1}&6 & 78 & 8 & 36 & 27.4 & 28 & 25 &\\
&& \ref{rec2}& 6 & 72 & 8 & 47 & 25.2 & 27 & 22 &\\
\bottomrule
\end{tabular}
\caption{C-\alg\ Results. Times are measured in millseconds.}\tablabel{learn}
\end{table}
%\end{wrapfigure}




==> status.tex <==
\section{Work: Status}

\paragraph{Where we aim to}
\begin{compactitem}
  \item Functions.
  \item More complicated basic formulas.
\end{compactitem}


==> synthesis-example.tex <==

\begin{table}[t]
\small
\ra{1.2}
\begin{tabular}{p{.15cm}p{1.7cm}p{.2cm}p{1.9cm}p{1.8cm}}\toprule
Line &~~Region & P &~~~Explanation & Regions \\  \midrule
1 &$[$-$\infty,\infty]$&$p_3$&Highest point & $[-\infty,p_3 $-$ 1]$, $[p_3 $+$ 1,\infty]$ \\
2 &$[p_3 $+$ 1,\infty]$&$p_5$&Highest point & $[p_3 $+$ 1, p_5 $-$ 1]$, $[p_5 $+$ 1,\infty]$ \\
3 &$[p_5 $+$ 1,\infty]$&$p_6$&Only point  & Empty \\
4 &$[p_3 $+$ 1,p_5 $-$ 1]$&$p_4$&Only point & Empty \\
5 &$[$-$\infty,p_3 $-$ 1]$&$p_1$&Highest point & $[-\infty, p_1 $-$ 1]$, $[p_1 $+$ 1,p_3 $-$ 1]$ \\
6 &$[p_1 $+$ 1,p_3 $-$ 1]$ &$p_2$&Only point & Empty \\
7 &$[$-$\infty, p_1 $-$ 1]$&$p_0$&Only point & Empty \\
\bottomrule
\end{tabular}
\caption{Head and Shoulders Synthesis Running Example.}\tablabel{overview:synthesisexample}\vspace{0.5cm}
\end{table}

